Default Bayes Factors for Testing the (In)equality of Several Population Variances

Testing the (in)equality of variances is an important problem in many statistical applications. We develop default Bayes factor tests to assess the (in)equality of two or more population variances, as well as a test for whether the population variances equal a specific value. The resulting test can be used to check assumptions for commonly used procedures such as the $t$-test or ANOVA, or test substantive hypotheses concerning variances directly. We show that our Bayes factor fulfills a number of desiderata. Researchers may have directed hypotheses such as $\sigma_{1}^{2} > \sigma_{2}^{2}$, they may want to extend $\mathcal{H}_{0}$ to have a null-region, or wish to combine hypotheses about equality with hypotheses about inequality, for example $\sigma_{1}^{2} = \sigma_{2}^{2} > (\sigma_{3}^{2}, \sigma_{4}^{2})$. We extend our Bayes factor test to allow for these deviations from our proposed default and illustrate it on a number of practical examples. Our procedure is implemented in the R package $bfvartest$.

==> ArXiv-Submission 2/shortcuts.tex <==
% REFERENCES --------------------------------------------------------------------------------------------------
%
\newcommand{\refFig}[1]{Fig.~{\ref{#1}}}
\newcommand{\refEq}[1]{Eq.~{\eqref{#1}}}
\newcommand{\refTab}[1]{Table~{\ref{#1}}}
\newcommand{\refSec}[1]{Section~{\ref{#1}}}
\newcommand{\refLem}[1]{Lemma~{\ref{#1}}}
\newcommand{\refCor}[1]{Corollary~{\ref{#1}}}
\newcommand{\refThm}[1]{Theorem~{\ref{#1}}}
\newcommand{\refEx}[1]{Example~{\ref{#1}}}
\newcommand{\refDef}[1]{Definition~{\ref{#1}}}
\newcommand{\refApp}[1]{Appendix~{\ref{#1}}}


\newcommand{\bibOrder}[1]{}

% MATHEMATICAL FIELDS --------------------------------------------------------------------------------------
%
\newcommand{\field}[1]{\mathbb{#1}} % the font for a mathematical field is blackboard
\newcommand{\R}{\field{R}} % the field of the reals
\newcommand{\N}{\field{N}} % the field of the natural numbers
\newcommand{\C}{\field{C}} % the field of complex number
\newcommand{\Z}{\field{Z}} % the field of integers

% LETTERS ---------------------------------------------------------------------------------------------------------
%
\newcommand{\1}{\mathbf{1}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Af}{\mathbb{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Bk}{\mathfrak{B}}
\newcommand{\Bf}{\mathbb{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ck}{\mathfrak{C}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Df}{\mathbb{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Ef}{\mathbb{E}}
\newcommand{\Ff}{\mathbb{F}}
\newcommand{\Fn}{\mathbb{F}_{n}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Gf}{\mathbb{G}}
\newcommand{\Gn}{\mathbb{G}_{n}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Kf}{\mathbb{K}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Lf}{\mathbb{L}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\Mnc}{\mathcal{M} \mathcal{N}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Nn}{N_{n}}
\newcommand{\Oc}{\mathcal{O}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Pf}{\mathbb{P}}
\newcommand{\Pn}{\mathbb{P}_{n}}
\newcommand{\Ps}{\mathscr{P}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\Qf}{\mathbb{Q}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Uc}{\mathcal{U}}
\newcommand{\Uf}{\mathbb{U}}
\newcommand{\Vc}{\mathcal{V}}
\newcommand{\Wc}{\mathcal{W}}
\newcommand{\Wf}{\mathbb{W}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Xf}{\mathbb{X}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Zc}{\mathcal{Z}}

% DERIVATIVE ---------------------------------------------------------------------------------------------------
%
\newcommand{\der}{\mathrm{d}}

% DISTRIBUTIONS ----------------------------------------------------------------------------------------------
%
\newcommand{\iid}{\textnormal{iid}}

\newcommand{\Ber}{\textnormal{Ber}}
\newcommand{\Bin}{\textnormal{Bin}}
\newcommand{\Pois}{\textnormal{Pois}}
\newcommand{\Gam}{\textnormal{Gam}}
\newcommand{\Beta}{\textnormal{Beta}}
\newcommand{\SBeta}{\textnormal{SBeta}}
\newcommand{\BetaPrime}{\textnormal{Beta2}}
\newcommand{\Dir}{\textnormal{Dir}}
\newcommand{\IG}{\textnormal{IG}}
\newcommand{\NIG}{\textnormal{NIG}}
\newcommand{\GIG}{\textnormal{GIG}}
\newcommand{\Exp}{\textnormal{Exp}}

% CONVERGENCE ------------------------------------------------------------------------------------------------
%
\newcommand{\as}{\overset{\textnormal{a.s.}}{\rightarrow}}
\newcommand{\inProb}{\overset{P}{\rightarrow}}
\newcommand{\inDist}{\overset{\textnormal{d}}{\rightarrow}}
\newcommand{\isDist}{\overset{\textnormal{d}}{=}}
\newcommand{\iidSim}{\overset{\iid}{\sim}}

% MATRICES -------------------------------------------------------------------------------------------------------
%
\newcommand{\Id}{\textnormal{Id}}
\newcommand{\Span}{\textnormal{Span}}
\newcommand{\tr}{\textnormal{tr}}

\newcommand{\la}{\langle} % Inner product: left
\newcommand{\ra}{\rangle} % Inner product: right

\newcommand{\inn}[2]{ \ensuremath{ \langle #1, #2 \rangle}}

\newcommand{\norm}[1]{ \ensuremath{ \| #1 \| }}


% OPERATORS -------------------------------------------------------------------------------------------------------
%
\newcommand{\convolution}{\ast}         % convolution
\DeclareMathOperator{\diag}{diag}       % een eigen wiskundeoperator
\DeclareMathOperator{\beeld}{Im}        % eigen wiskundeoperator
\DeclareMathOperator{\vecOp}{vec}
\DeclareMathOperator*{\plim}{plim}

% VARIANCE -----------------------------------------------------------------------------------------------------------
%
\newcommand{\var}{\textnormal{Var}}
\newcommand{\cov}{\textnormal{Cov}}
\newcommand{\cor}{\textnormal{Cor}}

% SUMS OF SQUARES and ERRORS -----------------------------------------------------------------------
%
\newcommand{\rss}{\textnormal{RSS}}
\newcommand{\ess}{\textnormal{ESS}}
\newcommand{\tss}{\textnormal{TSS}}
\newcommand{\mise}{\textnormal{MISE}}

% INFORMATION CRITERIA ---------------------------------------------------------------------------------
%
\newcommand{\Aic}{\textnormal{AIC}}
\newcommand{\Bic}{\textnormal{BIC}}
\newcommand{\Mdl}{\textnormal{MDL}}


% BAYES FACTORS -----------------------------------------------------------------------------
%
\newcommand{\BF}{\textnormal{BF}}
\newcommand{\LR}{\textnormal{LR}}
\newcommand{\info}{\textnormal{info}}
\newcommand{\bc}{\textnormal{BC}}
\newcommand{\elpdLoo}{\textnormal{elpd}_{\textnormal{loo}}}


% Abbreviations --------------------------------------------------------------------------------------------------
%
\newcommand{\dOri}{d_{\textnormal{orig}}}
\newcommand{\dRep}{d_{\textnormal{rep}}}
\newcommand{\dAll}{d_{\textnormal{all}}}

\newcommand{\pOri}{p_{\textnormal{orig}}}
\newcommand{\pRep}{p_{\textnormal{rep}}}

\newcommand{\nAll}{n_{\textnormal{all}}}
\newcommand{\nOri}{n_{\textnormal{orig}}}
\newcommand{\nRep}{n_{\textnormal{rep}}}

\newcommand{\ori}{_{\textnormal{orig}}}
\newcommand{\rep}{_{\textnormal{rep}}}
\newcommand{\all}{_{\textnormal{all}}}

\newcommand{\nPlan}{n_{\textnormal{plan}}}
\newcommand{\mPlan}{m_{\textnormal{plan}}}
\newcommand{\eff}{\textnormal{eff}}


% SPECIAL FUNCTIONS ------------------------------------------------------------------------
%
\newcommand{\sign}{\textnormal{sign}}
\newcommand{\Erf}{\textnormal{Erf}}
%
\newcommand{\vect}[1]{{\ensuremath{\vec{\reflectbox{\ensuremath{#1}}}}}}

% HYPERGEOMETRIC FUNCTIONS
\newcommand{\iFi}[3]{ \ensuremath{ \, {_{1} F}_{1} \left ( #1 \, ; \,  #2 \, ; \, #3 \right )}}
\newcommand{\iiFi}[4]{ \ensuremath{ \, {_{2} F}_{1} \left ( #1, #2 \, ; \, #3 \, ; \,  #4 \right )}}
\newcommand{\AFi}[6]{ \ensuremath{ \, AF_{1} \left ( #1 \, ; \,  #2, #3 \, ; \,  #4 \, ; \, #5, #6 \right )}}

% Empirical process
\newcommand{\Gfn}[2]{ \ensuremath{\mathbb{G}_{#1}(#2)}}
% Indicator function
\newcommand{\ind}[1]{\mathbf{1} \left \{ #1 \right \}}

%\definecolor{nOrange}{RGB}{245,160,80}
%\definecolor{nOrange}{RGB}{255,194,10}
%\definecolor{nOrange}{RGB}{255,176,0}
%\definecolor{nBlue}{RGB}{12,123,220}
%\definecolor{nRed}{RGB}{220,50,32}

% COLOURS ------------------------------------------------------------------------------------
%
\definecolor{nRed}{RGB}{220,0,12}
\definecolor{nOrange}{RGB}{254,166,0}
\definecolor{nBlue}{RGB}{40,96,180}

\newcommand{\nRed}[1]{\textcolor{nRed}{#1}}
\newcommand{\nOrange}[1]{\textcolor{nOrange}{#1}}
\newcommand{\nBlue}[1]{\textcolor{nBlue}{#1}}
